Spend Bits Where Queries Look: KV Cache Vector Quantization with Attention-Preserving Transforms

Long-context LLM decoding reads the key-value (KV) cache at every step. Loading it takes longer than computing attention over it, so throughput is bandwidth-bound. Hence, reducing the cache size can raise both decoding speed and serving capacity. The challenge is to reduce cache size while preserving the attention products, keeping reconstruction cheap, and using a fixed per-token bit count. At two bits per element, the most competitive methods rely on orthogonal transforms. However, existing techniques are either data-oblivious or use the query statistics without deriving the transform from a distortion criterion. Moreover, they rely on transforms built on top of random or Hadamard rotations, which equalize variances across entries rather than compacting energy, and fixed-width scalar quantizers, which are suboptimal at low rates. In this paper, we formulate KV cache quantization as a transform coding problem in which distortion is the error in the attention products. We derive closed-form optimal transforms for keys and values from calibration statistics, under a high-resolution model. We show that the optimal key transform is not orthogonal and satisfies a generalized Parseval relation: the attention-aware distortion becomes mean-squared error (MSE) in the transform domain. Thus, we can use MSE-optimal vector quantizers applied directly to the transformed key coefficients. To meet the fixed-width layout requirement, we show that grouping coefficients into equal-volume partitions makes equal-size codebooks attain the variable-rate optimum under the same high-resolution model. At two bits per element, our method, termed NOVA-KV, recovers most of the long-context retrieval accuracy lost by scalar quantization methods at comparable throughput.

==> notation.tex <==
\usepackage[hyphens]{url}  % DO NOT CHANGE THIS
\usepackage{graphicx} % DO NOT CHANGE THIS
\urlstyle{rm} % DO NOT CHANGE THIS
\def\UrlFont{\rm}  % DO NOT CHANGE THIS
\usepackage{natbib}  % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
\usepackage{caption} % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
\frenchspacing  % DO NOT CHANGE THIS
%\usepackage{booktabs}
\usepackage{multirow}
\usepackage{booktabs}
% These are recommended to typeset algorithms but not required. See the subsubsection on algorithms. Remove them if you don't have algorithms in your paper.
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{amssymb}   % \mathbb
\usepackage{amsmath}   % equation environments, \operatorname
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\usepackage{mathtools} % optional, extends amsmath

\usepackage{amsthm}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\usepackage[table]{xcolor}
% palette colors assumed defined: brickred = C1121F
\definecolor{brickred}{HTML}{C1121F}
\colorlet{oursrow}{brickred!12}   % light tint for the highlighted row
\usepackage{tikz}
\usetikzlibrary{positioning, arrows.meta, fit, backgrounds, calc}
\definecolor{slate}{HTML}{3B4B6B}
\definecolor{brick}{HTML}{9C3D3D}
\definecolor{brickfill}{HTML}{F3E4E4}
\definecolor{grayline}{HTML}{888888}
\definecolor{grayfill}{HTML}{F0F0F0}
% ---- paper palette ----
\definecolor{molten}{HTML}{780000}
\definecolor{brickred}{HTML}{C1121F}
\definecolor{papaya}{HTML}{FDF0D5}
\definecolor{deepspace}{HTML}{003049}
\definecolor{steel}{HTML}{669BBC}

\colorlet{slate}{deepspace}          % arrows / structural lines
\colorlet{brick}{brickred}           % strong red outline (new blocks, forward arrows)
\colorlet{brickfill}{brickred!8!white} % near-transparent red fill
\colorlet{grayline}{deepspace}       % std-block outline
\colorlet{grayfill}{steel!18!white}  % std blocks -> faint steel (was gray)% These are recommended to typeset listings but not required. See the subsubsection on listing. Remove this block if you don't have listings in your paper.
\usepackage{newfloat}
\usepackage{listings}
\DeclareCaptionStyle{ruled}{labelfont=normalfont,labelsep=colon,strut=off} % DO NOT CHANGE THIS
\lstset{%
	basicstyle={\footnotesize\ttfamily},% footnotesize acceptable for monospace
	numbers=left,numberstyle=\footnotesize,xleftmargin=2em,% show line numbers, remove this entire line if you don't want the numbers.
	aboveskip=0pt,belowskip=0pt,%
	showstringspaces=false,tabsize=2,breaklines=true}
\floatstyle{ruled}
\newfloat{listing}{tb}{lst}{}
\floatname{listing}{Listing}

\DeclareMathOperator*{\argmin}{arg\,min\,}

% Method name (use \method{} in text)
\newcommand{\method}{NOVA-KV}
\DeclareMathOperator{\tr}{tr}
%
% Recommended for better-looking tables
\usepackage{booktabs}

%
% Keep the \pdfinfo as shown here. There's no need
% for you to add the /Title and /Author tags.
\pdfinfo{
/TemplateVersion (2027.1)
}

\newcommand{\ci}[2]{#1\,{\scriptsize$\pm$#2}}
\newcommand{\cib}[2]{\textbf{#1}\,{\scriptsize$\pm$#2}}

\DeclareMathOperator{\softmax}{softmax}

\newtheorem{theoremA}{Theorem}
\newtheorem{lemmaA}{Lemma}
\newtheorem{propositionA}{Proposition}
\newtheorem{corollaryA}{Corollary}

\renewcommand{\thetheoremA}{A.\arabic{theoremA}}
\renewcommand{\thelemmaA}{A.\arabic{lemmaA}}
\renewcommand{\thepropositionA}{A.\arabic{propositionA}}
\renewcommand{\thecorollaryA}{A.\arabic{corollaryA}}
\usepackage{enumitem}
\definecolor{oursred}{RGB}{252, 228, 228} 
